Assessing Privacy Risks from Feature Vector Reconstruction Attacks

In deep neural networks for facial recognition, feature vectors are numerical representations that capture the unique features of a given face. While it is known that a version of the original face can be recovered via "feature reconstruction," we lack an understanding of the end-to-end privacy risks produced by these attacks. In this work, we address this shortcoming by developing metrics that meaningfully capture the threat of reconstructed face images. Using end-to-end experiments and user studies, we show that reconstructed face images enable re-identification by both commercial facial recognition systems and humans, at a rate that is at worst, a factor of four times higher than randomized baselines. Our results confirm that feature vectors should be recognized as Personal Identifiable Information (PII) in order to protect user privacy.

==> Makefile <==
LATEX=latex
BIBTEX=bibtex
BIBFILE=references.bib
PAPER=reconstruct

TEXFILES = reconstruct.tex \
	intro.tex \
	priorwork.tex \
	metrics.tex \
	visual.tex \
	features.tex \
	combined.tex \
	conclusion.tex \
	appendix.tex \

EPSFIGS = \

EPSGRAPHS = $(wildcard figures/*.eps)

all:   $(PAPER).pdf

subdirs:
	$(MAKE) -C figure

bib:
	$(BIBTEX) (PAPER)

%.eps: %.fig
	fig2dev -L eps $< $@

$(PAPER).ps: $(PAPER).dvi
	dvips -Ppdf -Pcmz -Pamz -t letter -D 600 -G0 -f $(PAPER).dvi > $(PAPER).ps

#$(PAPER).pdf: $(PAPER).dvi
#	dvipdf $(PAPER).dvi

# if need to embed font
$(PAPER).pdf: $(PAPER).ps
	ps2pdf14 -dEmbedAllFonts=true -dPDFSETTINGS=/prepress $(PAPER).ps

$(PAPER).dvi: $(EPSFIGS) $(TEXFILES) $(BIBFILE)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX) $(PAPER)
	$(LATEX)  $(PAPER)

$(PAPER).blg: $(BIBFILE)
	$(LATEX)  $(PAPER)
	$(BIBTEX) $(PAPER)
	$(LATEX)  $(PAPER)

clean:
	/bin/rm -f *.dvi *.aux *.ps *~ *.log *.lot *.lof *.toc *.blg *.bbl *.pdf *.out


==> combined.tex <==
\section{Deanonymization Success: Combining Metrics 1 and 2}

\todo{Write this}
